Optimizing Streamlined Blockchain Consensus with Generalized Weighted Voting and Enhanced Leader Rotation

Streamlined Byzantine Fault Tolerant (BFT) protocols, such as HotStuff [PODC'19], and weighted voting represent two possible strategies to improve consensus in the distributed systems world. Several studies have been conducted on both techniques, but the research on combining the two is scarce. To cover this knowledge gap, we introduce a weighted voting approach on Hotstuff, along with two optimisations targeting weight assignment distribution and leader rotation in the underlying state replication protocol. Moreover, the weighted protocols developed rely on studies proving the effectiveness of a specific voting power assignment based on discrete values. We generalise this approach by presenting a novel continuous weighting scheme applied to the Hotstuff protocol to highlight the effectiveness of this technique in faulty scenarios. We prove the significant latency reduction impact of weighted voting on streamlined protocols and advocate for further research.

==> experimental_setup_and_results.tex <==
\section{Evaluation} \label{experiements_results}

This paper analyses the impact of weighted voting on streamlined algorithms by gathering data from multiple experiments to determine whether or not introducing the voting power assignment generates significant latency improvements. 

\textbf{Implemented protocols} We evaluate the performance of Weighted Hotstuff~(\cref{weighted-hotstuff}), Weighted Chained Hotstuff~(\cref{chained-weighted-hotstuff}) and their multiple optimisation variants to weigh up against those of basic and chained Hotstuff, which are considered baseline for the non-faulty environments. Latency of the basic protocols is obtained by running the prediction model of Weighted Hotstuff with all weights equal to $V_{normal} = 1$. 

\textbf{Faulty scenario} Given the importance of availability in distributed environments, we critically analyse the worst-case scenario of faulty replicas. Since streamlined protocols are part of the BFT family, the system would need at least $3f + 1 $ nodes to withstand $f$ failures. Thus, for a given network scenario, the $f$ replicas holding the highest voting power are considered malfunctioning for faulty simulations of the protocols. In this way, the recovery performance of different Weighted Hotstuff optimisations can be compared.

\textbf{Experimental setup} For running the latency prediction models, we use Python scripts to test the behaviour of protocols in a given network scenario. Hence, each experiment depends on the specified distributed environment. Moreover, the latency estimation algorithm for Weighted Hotstuff requires providing a set of weights. The algorithm's behaviour matches that of Best Assigned Weighted Hotstuff in case of optimal weight assignment. Consequently, the experiments are conducted by tailoring the weighting distribution to the network scenario. That is, data on the distance within all replicas is gathered, and the $f$ best and $f$ worst connected replicas are assigned $V_{max}$ voting power. 

To make the analysis reliable, experiments are conducted using real data collected from cloudping, a tool for latency monitoring of deployed AWS clusters~\cite{cloudping}. For the results presented later in this section, the following clusters were used: \textit{Cape Town (af-south-1), Hong Kong (ap-east-1), Canada (ca-central-1), London (eu-west-2) and Northern California (us-west-1)}. This choice of network setting supports the research of weighted voting efficacy on geographically distributed settings since it reflects the heterogeneity of wide area network (WAN) environments. Moreover, simulations were performed using a blockchain system with $f = 1$ and $\Delta = 1$ (having a total of $n = 5$ replicas). Since Hotstuff is a protocol that sets itself apart from the others in the BFT family by using a new leader in each view, the views represent a critical aspect of the influence of weighted voting. Thus, we vary the number of views by performing simulations for values from 5 to 20 with $step = 1$.

The latency prediction models depend on the values generated for latency vectors $L_x$. In real-life simulations, the latency at which the leader receives messages from each replica is influenced by two factors: distance from leader to replica, reflected in link latency and the payload of the transmitted data, namely message delay. To emulate the network behaviour properly, for a leader $i$, we create its corresponding latency vectors $L_x$ as follows: distance within clusters (for the link latency) plus an offset drawn from a uniform sample $U(0, 5)$ for $L_{new}$ (since new-view messages encapsulate the block proposal, whereas the rest have lower payload containing just hashes) and $U(0, 2)$ for the rest. If the link is fast enough, the message payload latency can be neglected. However, for a better analysis of weighted voting, we went for a uniform distribution with significantly lower values than the cluster latency. In this way, message complexity is considered without severely influencing the protocol's behaviour but with the perks of mocking the heterogeneity of real environments.


\textbf{Weighted Hotstuff}~\cref{fig:hotstuff} showcases the impact of weighted voting on Hotstuff. It is clear from this visual representation of latency performance that introducing weighted voting decreases the latency of running the streamlined blockchain algorithm. Compared with the Basic Hotstuff in which all weights are assigned equal voting power, Weighted Hotstuff exhibits around $7\%$ decrease in latency. Adding to the $V_{max}/V_{min}$ weight assignment, the Optimal Leader Rotation variant reduces latency by up to $10\%$. However, there is room for improvement as Best Assigned Weighted Hotstuff indicates almost $20\%$ latency decrease. Furthermore, by combining the two optimisation approaches, (Optimal Leader Rotation + Best Assigned) Weighted Hotstuff reveals around $25\%$ latency reduction. Hence, the prediction models developed on multiple protocol variants support the idea established in AWARE of introducing leader relocation and weight-tuning mechanisms for improving the performance of blockchain algorithms. 

The figures also show that the optimal leader rotation variant has the same latency as its underlying weight optimisation Hotstuff variant over multiple of $n$ views. That is a consequence of the simulation framework using a static network setting for the experiments conducted. Since for such a simulation consisting of a multiple of $n$ views, each replica is the leader for an equal amount of times, the cumulative latency over all the views is the same.

In any distributed environment, resilience against failures is critical. Hence, we also analysed the latency performance over multiple views in faulty conditions for the developed Weighted Hotstuff protocols. For considering the worst-case scenario, replicas with the highest weights are considered faulty, jeopardising faster consensus. In this way, we force the analysed streamlined algorithms to mimic their fallback scenario strategy.~\cref{fig:hotstuff faulty} shows the average latency per view of Weighted Hotstuff and its variants. Out of all, the (Optimal Leader Rotation + Best) Weighted Hotstuff performs the best. Conversely, Best and Continuous Weighted Hotstuff express their over-fitting nature by showcasing significantly higher fallback latency. Since these two variants optimise the weight assignment for a given network scenario, the system would inevitably take longer to recover from an idle actor. Additionally, they perform worse than Weighted Hotstuff and its leader rotation optimisation version under normal network conditions and far worse under faulty ones.

\begin{figure}[h]
    \includegraphics[width=0.5\textwidth]{resources/2024.06.19_19:02:40.pdf}
    \caption{Average latency per view in \textbf{Hotstuff} protocol variants with $f = 1, \Delta = 1$.}
    \label{fig:hotstuff}
\end{figure}

\begin{figure}[h]
    \includegraphics[width=0.5\textwidth]{resources/faulty_2024.06.19_19:02:40.pdf}
    \caption{Average latency per view in \textbf{Hotstuff} protocol variants for \textbf{faulty scenario}, $f = 1, \Delta = 1$.}
    \label{fig:hotstuff faulty}
\end{figure}

\textbf{Chain Weighted Hotstuff}~\cref{fig:chained hotstuff} showcases the impact of weighted voting on Chained Hotstuff. The figure highlights the warming up period of $n$ views and supports the research of weighted voting on streamlined algorithms with a $7\%$ latency improvement gained by just assigning weights. Furthermore, adding a leader rotation optimisation on top of it accounts for an additional $3\%$ decrease in latency. As presented in Weighted Hotstuff, its chained version follows the same trends, exhibiting an average latency per view with $20\%$ better than the baseline (basic Chained Hotstuff) and performing best with an up to $25\%$ reduction for the combined version of the two optimisations.

Focusing on faulty network conditions,~\cref{fig:chained hotstuff faulty} presents the average latency per view of variants of the weighted streamlined protocol when $f$ defective nodes are in the system. Following the same method as Weighted Hotstuff, the $f$ replicas holding the highest weights are considered faulty such that the worst-case scenario is analysed. Despite behaving similarly to its basic version, Chained Hotstuff shows major differences in its fallback behaviour. Best Assigned Weighted Chained Hotstuff has the lowest fallback latency. That is due to the communication pattern of the chained protocol. Because simulations are performed under a specific set of weights, Chained Hotstuff cannot overfit when optimising for best weight assignment since the pipelined block proposal mechanism heavily influences the algorithm performance. With voting quorums for multiple blocks in one view, some weight assignments might benefit the consensus of one block whilst requiring more time to gather messages for the other. Hence, the Best Chained Hotstuff has higher resilience against idle nodes. Furthermore, the Weighted and Optimal Leader Rotation Weighted Hotstuff have higher fallback latency but still within the expected limits of \SI{200}{\milli\second} delay, with the latter performing better under this faulty environment setting.



\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\textwidth]{resources/chained_2024.06.19_19:38:03.pdf}
    \caption{Average latency per view in \textbf{Chained Hotstuff} protocol variants, $f = 1, \Delta = 1$.}
    \label{fig:chained hotstuff}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\textwidth]{resources/chained_faulty_2024.06.19_19:38:03.pdf}
    \caption{Average latency per view in \textbf{Chained Hotstuff} protocol variants for \textbf{faulty scenario}, $f = 1, \Delta = 1$.}
    \label{fig:chained hotstuff faulty}
\end{figure}

\textbf{Continuous Weighting Scheme} The analysis of Continuous Weighted Hotstuff provided in~\cref{fig:hotstuff} and~\cref{fig:hotstuff faulty} highlight that its performance matches the one of Best Assigned Weighted Hotstuff. In the non-faulty case, it is clear that the continuous scheme achieves, at best, the same performance as the best weight distribution, but the faulty scenario is up for investigation. Given that the previous experiments were conducted on a fixed network setting, a further experiment on a randomly generated network topology with within clusters latency ranging between $0$ and \SI{400}{\milli\second} was performed.~\cref{fig:analysis_continuous_hotstuff} showcases the difference in latency between the Best Assigned and Continuous Weighted Hotstuff and proves that the latter performs better in $85\%$ of the performed simulations. Hence, the research supports further study of the continuous metric for voting power assignment. 

\begin{figure}[h]
    \centering
    \includegraphics[width=0.4\textwidth]{resources/continuous_2024.06.19_15:11:10.pdf}
    \caption{Best Assigned vs Continuous Weighted Hotstuff latency performance, $n = 5$, $10$ views executed.}
    \label{fig:analysis_continuous_hotstuff}
\end{figure}


\begin{table}[h]
\centering
\caption{Comparison of the average latency improvement of \textbf{Weighted Hotstuff} variants based on \cref{fig:hotstuff,fig:hotstuff faulty,fig:chained hotstuff,fig:chained hotstuff faulty}.}
\label{tbl:latency_improvement_table}
\small
\begin{tabular}{@{}lcc@{}}
\toprule
 & \textbf{Basic} & \textbf{Chained} \\
\midrule
\textbf{No optimisation}              & -7.13\%                    & -7.28\%    \\          
\textbf{Best Assigned}                  & -19.48\%                   & -19.64\% \\
\textbf{Optimal Leader Rotation}         & -10.52\%                   & -9.78\% \\           \textbf{Continuous}            & -18.30\%                   & n.a     \\          \textbf{Optimal Leader Rotation + Best Assigned}  & -24.36\%                   & -22.48\%   \\       
\bottomrule
  \end{tabular}
\end{table}

